Biodegradable Interactive Materials

The sense of touch is fundamental to how we interact with the physical and digital world. Conventional interactive surfaces and tactile interfaces use electronic sensors embedded into objects, however this approach poses serious challenges both for environmental sustainability and a future of truly ubiquitous interaction systems where information is encoded into everyday objects. In this work, we present Biodegradable Interactive Materials: backyard-compostable interactive interfaces that leverage information encoded in material properties. Inspired by natural systems, we propose an architecture that programmatically encodes multidimensional information into materials themselves and combines them with wearable devices that extend human senses to perceive the embedded data. We combine unrefined biological matter from plants and algae like chlorella with natural minerals like graphite and magnetite to produce materials with varying electrical, magnetic, and surface properties. We perform in-depth analysis using physics models, computational simulations, and real-world experiments to characterize their information density and develop decoding methods. Our passive, chip-less materials can robustly encode 12 bits of information, equivalent to 4096 unique classes. We further develop wearable device prototypes that can decode this information during touch interactions using off-the-shelf sensors. We demonstrate sample applications such as customized buttons, tactile maps, and interactive surfaces. We further demonstrate the natural degradation of these interactive materials in degrade outdoors within 21 days and perform a comparative environmental analysis of the benefits of this approach.

==> sections/_Archive/v1_2_related_work.tex <==
\section{Related Work \& Overview}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/Overview.png}
    \caption{Overview}
    \label{fig:overview}
\end{figure*}

This interdisciplinary work builds on classic physics, sustainable materials, fabrications, sensing, and ubiquitous computing. There is no previous work similar to our proposed concept of \textit{interactive material}. So we present the relevant works that motivated the goals of this work below, especially in computational materials \cite{abowd_internet_2020}.

Our initiative is motivated by the vision articulated by Gregory Abowd's vision talk at the UIST 2018, "Advances in materials science and manufacturing today signal a time when we really will be able to manufacture new everyday materials that have computational capabilities 'woven' into them". He introduced the notion of the Internet of Materials (IoM)  \cite{abowd_internet_2020} as an evolution beyond the well-known concept of the Internet of Things (IoT). He envisioned a future where "everyday objects made of everyday materials with the ability to behave as connected computational entities", these new and functional materials are termed "computational materials".

Despite the motivation and potential heralded by Abowd's vision, the reality, six years on, only a few works \cite{arora_saturn_2018,arora_mars_2021} meet his expectation for \textit{self-sustainable computational materials}. Most research had only focused on innovating the traditional IoT devices to be battery-free through the integration of energy-harvesting modules--- using photovoltaic or solar cells \cite{zhang_optosense_2020, zhang_flexible_2022, waghmare_ubiquitouch_2020, de_winkel_battery-free_2020}, piezoelectric generator \cite{lu_battery-less_2020, jang_underwater_2019}, or NFC \cite{kim_remote_2023} to replace conventional batteries. These works, while improved, fall short of achieving the transformative leap toward IoM.

The gap between the current state of technology and the envisioned future of IoM underscores the significant challenges involved in creating computational objects that simultaneously address self-sustainability in terms of power and life cycle, manufacturing scalability, and capability of mimicking the form factors of physical objects we interact with daily. It prompts a moment of reflection: Could we, perhaps, recalibrate our ambitions and explore the creation of interactive materials as a stepping stone toward computational materials?

This reimagined approach is further inspired by the recent work on the Internet of Bioinspired Things \cite{iyer_wireless_2020, iyer_wind_2022, johnson_solar-powered_2023}, can we create interactive materials through the exploration of how nature’s entities, from honeybees to sea turtles and spiders, interact with their environment through innate mechanisms. These natural phenomena, although not "computational" in the sense of von Neumann architecture (used in today's modern computing and digital devices), offer a rich tapestry of ideas for our design of interactive materials (\textcolor{blue}{Figure~\ref{fig:overview}}).

% Honeybees, produce sensory hairs to perceive the electrical field, so they can sense the alternation of the electric field surrounding flowers to determine if the flower has been recently visited, i.e., nectar availability; Sea turtles can detect magnetic field's intensity and inclination, so they utilize the Earth's magnetic field to discern their latitude; spiders have slit sensillae, a form of mechanical receptor capable of detecting minute vibrations and surface irregularities, so they can discern varied terrains for web placement and vibrations traveling through their webs for prey hunting. Such natural phenomena are highly attractive for creating interactive materials: can we leverage the natural physical property of every material as a medium for information encoding? 

\subsection{Sustainable Material Selection}
The urgency of sustainability permeates across disciplines, resonating strongly within the HCI community against the backdrop of the broader societal shift towards environmental consciousness. Yet, the path to ultimate sustainable computing is fraught with complexities, as evidenced by many recent works that used water-soluble plastic such as polyvinyl alcohol (PVA) \cite{cheng_functional_2023} but claimed "sustainable". However, these water-soluble plastics, while dissolving in water, do not disintegrate in the ecological sense; their chemical constituents persist, and complete biodegradation is contingent upon specific environmental conditions rarely met even in the wastewater treatment systems \cite{rolsky_degradation_2021}.

The most exciting research recently in sustainable computing has been directed toward the development of bio-based \cite{vasquez_myco-accessories_2019, koelle_prototyping_2022, nicolae_biohybrid_2023} and recyclable materials \cite{zhang_recyclable_2023} for circuits, aiming to extend the lifecycle of electronic components while circumventing the environmental pitfalls associated with processing the raw material of traditional bioplastics. Despite these advances, such biomaterials are often compromised by their inherent heterogeneity and non-cohesive morphologies, resulting in suboptimal mechanical properties and challenging processability issues, rendering them impractical for making everyday objects.

Addressing these challenges, in this work, we capitalize on the recent development of creating backyard-compostable bioplastics from raw microalgae \cite{campbell_progress_2023}, with a simple and scalable fabrication methodology such as heat pressing  \cite{iyer_fabricating_2023} and 3D printing \cite{fredricks_spirulina-based_2021}. These techniques yield materials with mechanical properties comparable to those of conventional plastic filaments. As a proof of concept, we select chlorella (a type of algae) as the base material, along with graphite and magnetite (a natural mineral) to tune the material properties. We imagine the future of sustainable materials extracted from renewable biological matter and processed through eco-friendly techniques to minimize environmental burdens.


\subsection{Sustainability-driven Sensing Design Considerations}

\begin{table*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/LCAComparison_Main_v2.png}
    \caption{LCA Comparison}
    \label{tab:LCAComparison_Main}
\end{table*}

In addition to prioritizing sustainable materials, our design philosophy extends to optimizing sustainability in our sensing approach. Sensing interactions (e.g., touch detection) traditionally fall into two categories: integrating sensors within physical interfaces, including capacitive \cite{sato_touche_2012, holloway_accessible_2018, cheng_swellsense_2023} and vibration sensors \cite{arora_saturn_2018, chen_reviving_2017}, or embedding these sensing capabilities into wearable devices \cite{waghmare_z-ring_2023}.

The burgeoning IoT industry, with its exponential growth rate of billions of new devices every year \cite{daepp_eclipse_2022}, exemplifies the logistical and environmental challenges posed by embedded sensing mechanisms in physical interfaces. Such sensing approach for interactive material, while effective, risks compounding the already significant issue of e-waste. To circumvent these potential environmental repercussions, our strategy favors wearable device-based sensing. This choice is predicated on several advantages that align with sustainable practices: firstly, it centralizes the sensing mechanism, reducing the quantity of electronics per user to a single wearable device. This reduction is crucial for minimizing waste. Secondly, the personal nature of wearables facilitates better end-of-life treatment and power management, including the option to activate the device only when needed, thereby minimizing unnecessary power consumption power. 

Our cradle-to-grave environmental impact comparison in \textcolor{blue}{Table~\ref{tab:LCAComparison_Main}} (see \textcolor{blue}{Table A\ref{tab:LCAComparison_1}\&\ref{tab:LCAComparison_n}} for detailed comparisons of scenarios involving single and multiple interactive interfaces) juxtaposes our biodegradable interactive materials with the wearable-based sensing strategy against traditional methods involving 3D-printed physical interfaces equipped with embedded capacitive sensing circuits. This comparison leverages the recent concept in comparative life-cycle assessment \cite{zhang_deltalca_2024} to underscore the environmental benefits of our approach.

In the subsequent sections, we delineate the creation of interactive materials utilizing three inherent material properties. An overview of these material properties and their associated sensing technologies is illustrated in \textcolor{blue}{Figure~\ref{fig:overview}}. For each material property explored, we leverage commonly available sensors (e.g., impedance sensors, magnetometers, microphones) for information decoding. This decision to utilize off-the-shelf sensors, rather than developing custom sensors, is informed by two practical considerations that may throttle the pace of further innovation in interactive material: 1) custom sensors often incur prohibitive fabrication costs and times, making replication inaccessible to researchers in the broader HCI community; 2) sensors tailored for specific purposes may have difficulty adapting to new material properties or scenarios.

Through these considerations, our approach not only adheres to our principles of sustainable computing but also paves the way for the ubiquitous deployment of interactive materials.

==> sections/_Archive/v1_3_conductivity.tex <==
\section{Electrical Properties}
In the exploration of creating interactive materials through the lens of conductivity, our inspiration is drawn from the natural world. Animals have evolved various mechanisms to use electroreception to interact with or navigate nature. Platypuses, produce bills with electroreception to detect the electric fields generated by the muscular contractions of their prey; honeybees, produce sensory hairs to perceive the electrical field surrounding flowers. Honeybees accumulate positive charges while flying while flowers gain negative charges through electrostatic induction. The interaction between honeybees and flowers alters the electric field of the flowers, this alteration, with information about the flower has been recently visited, i.e., nectar availability could be perceived by other honeybees before landing. Such natural phenomena are highly attractive for creating interactive materials: conductivity could not just be a physical property but a medium for information encoding and sensing. 

Building on this, in this section, we aim to encode information into materials through conductivity and extend human sensory capabilities by leveraging the recent development of wearable bio-impedance sensing technology \cite{waghmare_z-ring_2023, zhang_advancing_2016, jung_wrist-wearable_2021}. Our approach aims to replicate, in human users, a bee-like ability to discern and interact with the electrical properties of their surroundings. 

\subsection{Theory}
The foundational premise of employing material conductivity $\sigma$ to encode information and its decoding through wearable bio-impedance sensors is rooted in an amalgam of classical electrical theory and contemporary bioelectrical impedance analysis. We explain the backbone of this conceptual framework using elements of a simplified circuit model that encapsulates the interaction between the user and the interactive materials. 

We assume that the user's finger and the external surface form a series connection upon contact, the system's total impedance, $Z_{total}$, manifests as the sum of the finger's bio-impedance $Z_{bio}$, the contact electrical impedance $Z_{contact}$, and the inherent material impedance $Z_{material}$, mathematically represented as:
\begin{equation}
   Z_{total} = Z_{bio} + Z_{contact} + Z_{material}
\label{eq:Z_total}
\end{equation}

Bio-impedance, a measure of biological tissues' opposition to electric current, varies with tissue type and state, such as hydration. In our case, we neutralize the variable of the user's inherent bio-impedance by only focusing on the change in impedance $\Delta Z$ upon contact with an external surface, i.e., the add-in impedance of interactive material and contact:
\begin{align}
    \Delta Z &= Z_{total,new} - Z_{total,initial} \nonumber \\
    \Rightarrow \Delta Z &= (Z_{bio} + Z_{contact} + Z_{material}) - Z_{bio} \nonumber \\
    &= Z_{contact} + Z_{material}
\label{eq:delta-Z}
\end{align}


\subsubsection{Contact Impedance}
Our theoretical framework made the following simplifying assumptions:
\begin{enumerate}
    \item Contact surfaces are clean without insulating barriers, as well as continuous and frictionless.
    \item There is no tensile stress at the contact point.
    \item User's finger is a perfectly elastic solid and skin surface is smooth, i.e., no friction ridges and lines; external interactive material surface is a perfectly rigid body.
\end{enumerate}

Under these conditions, $Z_{contact}$ is governed by the resistivity, and the size of the contact radius relative to the electron mean free path, which transitions between Sharvin and diffuse scattering mechanism, as explained in the Maxwell spreading resistance formula \cite{wexler_size_1966}:
\begin{equation}
    Z_{contact} = \frac{4\rho^{*} l_{e}}{3\pi a^{2}} + v\left(l_{e}/a\right)\frac{\rho^{*}}{2a}
\label{eq:Wexler}
\end{equation}
where $\rho$ is the resistivity separating two bodies, $l_{e}$ is the electron mean free path length of the material, $a$ is the contact radius, $v$ is a function of the ratio $l_{e}/a$, and $\rho^{*}$ is $\frac{\rho_1+\rho_2}{2}$, $\rho_1, \rho_2$ are the resistivity on two sides of the contact, respectively. Given the dominance of the diffuse scattering mechanism in our context $a \gg l_{e}$, so that
\begin{align}
    \lim\limits_{{l_e}/a \to 0} v\left({l_e}/a\right) &= 1 \nonumber \\
    \frac{4\rho^{*} l_{e}}{3\pi a^{2}} &\approx 0 \nonumber 
\label{eq:le/a}
\end{align}
Now Eq.\ref{eq:Wexler} can be simplified to
\begin{equation}
    Z_{contact} = 0 + 1\times\frac{\rho^{*}}{2a} = \frac{\rho^{*}}{2a} \Leftrightarrow \frac{\rho_{finger}+\rho_{material}}{4a}
\label{eq:Wexler_simplified}
\end{equation}

\paragraph{Hertzian Contact Stress Model} This relationship is further refined through the Hertzian contact stress model, accounting for the applied force and the elastic properties of the finger and interactive material, to express the effective contact radius of the finger pad $a$ and, consequently, the contact area $A$. For contact radius $a$, we have
\begin{equation}
    a = \left[ \frac{3FR^{*}}{4E^{*}} \right]^{\frac{1}{3}}
\label{eq:Hertzian}
\end{equation}
where $F$ is the force applied over the contact area of the finger and material surface, $R^{*}$ is the effective radius of curvature of the finger and material surface, and $E^{*}$ is the effective modulus of elasticity of the system. $R^{*}$ is defined as
\begin{equation}
    \frac{1}{R^{*}} = \frac{1}{R_{finger}}+\frac{1}{R_{material}} 
\label{eq:effective_radius}
\end{equation}

Since we assume the external interactive material surface is a perfectly rigid body, for a rigid surface, its radius of curvature $R_{material}$ can be considered infinitely large:
\begin{align}
    \lim\limits_{R_{material} \to \infty} \left(\frac{1}{R_{finger}}+\frac{1}{R_{material}} \right) &= \frac{1}{R_{finger}} \nonumber \\
    \Rightarrow \frac{1}{R^{*}} = \frac{1}{R_{finger}} \Leftrightarrow R^{*} &= R_{finger}
\label{eq:effective_radius_2}
\end{align}

By incorporating the mechanics of contact between disparate materials, specifically between a sphere (i.e., the user's finger) and a flat surface (i.e., the material). We define the effective modulus of elasticity $E^{*}$ as a function of the individual modulus of elasticity $E$ and Poisson ratios $v$ of the interacting bodies. This relationship is quantified as follows
% cite https://ece.northeastern.edu/edsnu/mcgruer/thesis/SumitMajumder/chap2_revi.pdf
% https://wp.optics.arizona.edu/optomech/wp-content/uploads/sites/53/2016/10/Tutorial_Etter-Jacob.pdf
\begin{equation}
    \frac{1}{E^{*}} = \frac{3}{4} \times \left( \frac{1-{v_{finger}}^{2}}{E_{finger}}+\frac{1-{v_{material}}^{2}}{E_{material}} \right)
\label{eq:elasticity}
\end{equation}

Given the substantially higher modulus of elasticity for rigid object surfaces compared to elastic biological tissues, $E_{material} \gg E_{finger}$, therefore Eq.\ref{eq:elasticity} can be simplified with the material's contribution becoming negligible:
\begin{equation}
    \Rightarrow \frac{1}{E^{*}} \approx \frac{3}{4} \times \frac{1-{v_{finger}}^{2}}{E_{finger}}
\label{eq:elasticity_2}
\end{equation}

This leads us to a simplified Hertzian contact stress model from Eq. \ref{eq:Hertzian}, which allows us to calculate the contact radius $a$ considering the force applied during the touch interaction and the inherent physical properties of the finger:
\begin{equation}
    a = \left[ \frac{9F R_{finger}} {16 \left( \frac{E_{finger}}{1-{v_{finger}}^{2}} \right)} \right]^{\frac{1}{3}}
\label{eq:Hertzian_final}
\end{equation}

% \begin{equation}
%     A = \pi a \xi = \pi\left[ \frac{9FR_{finger}} {16 \left( \frac{E_{finger}}{1-{v_{finger}}^{2}} \right)} \right]^{\frac{2}{3}}
% \label{eq:contact_area }
% \end{equation}

In validating our theoretical contact stress model of the finger and interactive material, empirical results from recent studies characterizing human skin tissue and finger mechanics are used: a Poisson ratio for human skin tissue of 0.48 \cite{li_determining_2012}; an average tap force of 0.50 N with a standard deviation of 0.09 N \cite{asakawa_fingertip_2017}; the elasticity of the finger, as characterized by Young’s modulus, presents a wide range due to factors such as applied normal load, gender differences, and the anatomical variance between the skin's superficial and deeper layers adjacent to the bone, fluctuating between 0.2 MPa \cite{oprisan_experimental_2016} and 4.6 MPa \cite{pawlaczyk_age-dependent_2013}. For the purposes of our analysis, the effective curvature radius of the finger is approximated as 1 cm. Substituting these empirically derived values into our final Hertzian contact stress model Eq.\ref{eq:Hertzian_final}, we derive the effective contact radius: 
\begin{align}
    % a &= \left[ \frac{9\cdot0.5N\cdot0.01m} {16 \left( \frac{E_{finger}}{1-{0.48}^{2}} \right)} \right]^{\frac{1}{3}}, E_{finger}\in [0.2 MPa, 4.6 MPa] \nonumber \\
    a &\in [0.84 mm, 2.40 mm]
\label{eq:radius_number}
\end{align}

These results align with empirical observations---19.9 and 14.0 mm for the orientations of 30° and 45° \cite{dzidek_contact_2017}. This stress model is a critical component in understanding the contact interface of tactile interactions. A study also characterized the resistivity of the living epidermis (the outermost layer of skin) of fingers to be 11 $\Omega \text{m}$ at 1 MHz \cite{tsai_dielectrical_2019}. By integrating these datums into Eq.\ref{eq:Wexler_simplified}, we derive the contact impedance, $Z_{contact}$, as a function of material resistivity:

\begin{equation}
    Z_{contact} = \frac{11 \Omega \text{m}+\rho_{material}}{4a}, a \in [0.84 mm, 2.40 mm]
\label{eq:Wexler_final}
\end{equation}

\subsubsection{Impedance of Interactive Material}

The intrinsic impedance $Z_{material}$ diverges in behavior under alternating current (AC) conditions, necessitating a distinction from direct current (DC) scenarios where impedance equates to resistance, $R$. In the AC paradigm, where common capacitive sensors and bio-impedance sensors operate at, $Z_{material}$ embodies both resistive and reactive components:
\begin{equation}
    Z_{material} = R+jX
\label{eq:Z_material}
\end{equation}
where $j$ is the imaginary unit and $X = \omega L - \frac{1}{\omega C}$, $\omega$ is the angular frequency $2\pi f$. Assume interactive materials as regular solid cuboids with constant area $A$ and thickness $t$ for simplification, we deduce expressions for resistance, $R = \rho \frac{t}{A}$, and capacitance, $C = \frac{t}{\omega \epsilon A}$. Due to the diamagnetism of common conductive materials such as copper, silver, and graphite, which results in low magnetic permeability, the inductance part could be negligible. Now we have Eq.\ref{eq:Z_material} as
\begin{equation}
    Z_{material} = \rho \frac{t}{A} - j\frac{t}{\omega \epsilon A} = \frac{t}{A} (\rho - j\frac{1}{\omega \epsilon})
\label{eq:Z_material_2}
\end{equation}

We know that in the theory of wave causality in classical electrodynamics, permittivity is a complex quantity and can be expressed as $\epsilon = \epsilon' + j\epsilon'' = \epsilon_0 + j \frac{\sigma}{\omega } \Rightarrow j\frac{1}{\omega \epsilon} = j\frac{1}{\omega  (\epsilon_0 + j \frac{\sigma}{\omega })} = \frac{-\omega }{j\omega^2 \epsilon_0 - \sigma}$. Thus, Eq.\ref{eq:Z_material_2} arrives at:

\begin{equation}
    Z_{material} = \frac{t}{A} (\frac{1}{\sigma} + \frac{\omega }{j\omega^2 \epsilon_0 - \sigma})
\label{eq:Z_material_3}
\end{equation}


\subsubsection{Final Impedance Change Model}
For the minimal dimensions of interactive material pixel, we adhere to Apple’s Accessibility Human Interface Guidelines \cite{apple_accessibility_nodate}, which suggest that a hit target should measure at least 44$\times$44 points, approximately 15$\times$15 mm. We envision our interactive materials being applied to the surface of everyday objects rather than filling the entire solid object. Consequently, they will be thin, such that $t\ll A$. Therefore, the impedance of the interactive material is negligible in our final calculation unless in a low-frequency region (e.g., $f<1kHz$), where the term $(\rho - \frac{1}{\omega \epsilon})$ is dominated by the permittivity. We thereby describe the impedance change Eq.\ref{eq:delta-Z} as: 
\begin{align}
     \Delta Z &= Z_{contact} + Z_{material} \approx Z_{contact} \nonumber \\
     &= \frac{11 \Omega \text{m}+\rho_{material}}{4a}, a \in [0.84 mm, 2.40 mm], f > 1MHz
\label{delta-Z-final}
\end{align}

% To ensure a good SNR or read margin between each possible conductivity state, we consider the varies in such as touch force and tissue properties between each touch and user as background noise or the region of uncertainty. We use the measured resistivity of chlorella ($1.86\times10^8 \Omega \text{m}$) as the upper bound (please refer to the subsequent section) and $\rho_{finger}$ ($11 \Omega \text{m}$) as the lower bound for the possible tuning range of $\rho_{mateiral}$, this is because if the interactive material has great conductivity, i.e., $\rho_{mateiral} \ll \rho_{finger}$, the contact resistance part will be dominated by $\rho_{finger}$. In that case, we could tune the size $A$ of the interactive material to encode information. However, surface pattern is a different property that will not be discussed in the section. Such that, by tuning the material conductivity, we are able to encode 

To optimize the signal-to-noise ratio (SNR) and read margin between each possible conductivity states, the variance in touch force and user-specific biological tissue properties are considered as background noise or the uncertainty region. We set the resistivity bounds of $\rho_{mateiral}$ from chlorella ($1.86\times10^8 \Omega \text{m}$, please refer to Section 3.3) to $\rho_{finger}$ ($11 \Omega \text{m}$). This delineation is predicated on the principle that if the interactive material exhibits superior conductivity like copper (i.e., $\rho_{material} \ll \rho_{finger}$), then the contact resistance part will be dominated by $\rho_{finger}$. Under such circumstances, the dimension—specifically, the area ($A$) of the interactive material—becomes a tunable parameter for encoding information, however this is a different material property and will not be discussed here. In conclusion, by tuning the conductivity of the material, it becomes feasible to encode information within a spectrum of approximately 32 discrete states, equivalent to 5 bits of data, as expressed by the following equation:

\begin{equation}
    \log_{1.68}{(1.86\times10^8 \Omega \text{m} \div 11 \Omega \text{m})} \approx 32 \text{ states} \Leftrightarrow \log_{2}{32} = 5 \text{ bits}
    \label{eq:conductivity_result}
\end{equation}

Through this theoretical exposition, our objective is not only to elucidate the boundaries of information encoding within materials via conductivity but also to outline the mechanism by which a wearable impedance sensor could decode this information.

% highlights the sensitivity of the system to variations in mechanical properties of the human skin and the applied force, underscoring the complexity of encoding information through conductivity in interactive materials.

% S11:
% \begin{equation}
%     S11 = \frac{Z_{L} - Z_{0}}{Z_{L} + Z_{0}}
% \label{eq:s11}
% \end{equation}

\subsection{Simulation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Conductivity_simulation_v2.png}
    \caption{a, CST simulation setup. b, CST simulation S11 results. c, pitch angle sweep.}
    \label{fig:conductivity_simulation}
\end{figure*}
Before transitioning from theory to real-world validations, the employment of FIT simulation is an indispensable intermediary in the iterative design process, as it provides a controlled environment to test our hypotheses regarding material conductivity and its decoding through wearable impedance sensors.

In our specific study, the simulation is conducted using the Simulia CST Studio Suite, leveraging its 3D electromagnetic (EM) analysis capability. We determine the frequency range of 1 MHz to 500 MHz for our simulations, drawing on recent findings highlighting a significant attenuation of specific absorption rate (SAR) dynamics within human tissue beyond 500 MHz \cite{waghmare_z-ring_2023}.

We constructed a bio hand model representative of a 38-year-old male, 180 cm in height and 103 kg in weight, utilizing the CST Bio Models Library and the US National Library of Medicine's Visible Human Project. Our model incorporates 31 distinct tissue types at a resolution of $1\times1\times1 \text{mm}$, and isolates the right hand from the rest of the body tissues to reduce the size of mesh volume and computation complexity. The bio-impedance measurement point is set at the proximal phalange (the common position to wear a ring-form-factor device) of the index finger (the common finger to touch an external object). 

The interactive materials are created with dimensions of $20\times20\times5 \text{mm}$, balancing the requirements for minimal accessible touch size and interactive material 'pixel' density. Within this framework, conductivity emerges as the sole variable, with all other material properties, such as loss tangent, held constant to isolate the effect of other contributions. The simulation models the contact interface between the fingerpad and interactive materials, following our calculation in Eq.\ref{eq:radius_number} of contact radius and pressure distribution. The final model setup is illustrated in \textcolor{blue}{Figure~\ref{fig:conductivity_simulation}a}.

% Our RF simulation is conducted using the Simulia CST Studio Suite. We created the bio hand model from the CST Bio Voxel Models Library. The tissue properties of a 38-year-old male, 180 cm in height, 103 Kg are used. The voxel model contains 31 tissues with a resolution of 1x1x1 mm. The final bio hand model setup is shown in \textcolor{blue}{Figure~\ref{fig:}}, we keep the right hand and remove the rest of the body to reduce the size of the mesh volume and computation complexity. We set the bio-impedance measurement point at the proximal phalange, the most common place to wear a ring form factor device, of the index finger, the most common finger for right-handed to touch an external object. We designed the interactive materials in the dimensions of 20 x 20 x 1 mm to adhere both minimal 'pixel' size and the minimal size for hit target. We keep the other parameters of the material, such as permittivity, constant, and set the conductivity as the only variable. We created the contact between the fingerpad and the interactive material following our calculation in Eq.\ref{eq:radius_number}.

To explore the conductivity spectrum of the interactive materials, we conduct a logarithmic parameter sweep from $5.37\times10^{-9}$ S/m to $6.87\times10^{-7}$ S/m with a total of 8 samples. This interval selection is predicated on the minimal read margin calculated in Eq.\ref{eq:conductivity_result} to achieve a good SNR, ensuring discernible differentiation between each conductive state. Each parameter value required approximately 100 minutes for simulation on a 14-core CPU and a single RTX 4070Ti GPU. The measurements of S11, also known as the reflection coefficient, are used to determine the impedance. S11 is a metric that specifies the amount of a wave reflected by the impedance mismatch in the transmission medium, defined as the ratio of the reflected wave’s amplitude to the incident wave’s amplitude. The simulation results reveal macroscopic distinctions across 8 conductivity levels as shown in \textcolor{blue}{Figure~\ref{fig:conductivity_simulation}b}, corroborating our theoretical predictions.

Further examination extends to the influence of finger orientation on touch interaction. We perform another linear parameter sweep of touch pitch angles from -20 degrees to +20 degrees with a total of 5 samples onto the existing model. The S11 simulation results, along with the nearest conductivity states as references, are shown in \textcolor{blue}{Figure~\ref{fig:conductivity_simulation}c}, revealing the robustness of conductivity detection across a range of touch orientations. The aggregation of these 3D EM simulation results validates our theoretical constructs.

%https://space.mit.edu/RADIO/CST_online/mergedProjects/3D/common_tools/common_tools_biomodels.htm


\subsection{Implementation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Conductivity_measurement.png}
    \caption{a, conductivity (N>=3). b, flexural strength Ultimate tensile strength (N>=5). c, real-world measurement.}
    \label{fig:conductivity_implementation}
\end{figure*}

Having substantiated our hypothesis through both theoretical articulation and simulation insights, we now transition to the tangible implementation. This phase entails the fabrication of interactive materials with varied conductivities, alongside the development of a wearable sensor system capable of decoding this conductivity. We aim to validate the feasibility of our approach in encoding information within materials through their inherent conductivity properties in practice.

We fabricate the interactive material with different conductivities by mixing chlorella with varying proportions (0\%--28\%) of graphite or magnetite Fe3O4. Graphite, is a crystal allotrope of carbon, exhibiting good electric conductivity due to the delocalized $\pi$-electrons between carbon hexagonal lattice layers; Magnetite, a natural mineral of iron ores, exhibits electrical conductivity attributed to electron exchange between iron ions in different oxidation states within the crystal lattice.

We first characterize the conductivity of the fabricated samples (see \textcolor{blue}{Section \ref{Resistivity}} for details), revealing a direct positive correlation between the addition of conductive materials and enhanced conductivity. The results are shown in \textcolor{blue}{Figure~\ref{fig:conductivity_implementation}a}. We note that graphite's inclusion resulted in a more pronounced increase in conductivity compared to magnetite, reflective of its superior electrical properties (graphite: $3.3\times10^2$ to $2\times10^5$ S/m, magnetite: 0.1 S/m). We observe a stark rise in conductivity between graphite concentrations of 5\% to 8\%, marking the percolation threshold--- a point at which our interactive material transitions from a nearly insulator to a conductor due to the formation of a continuous path for electron flow. The resistivity and conductivity of pure chlorella are characterized at $1.86\times10^8 \Omega \text{m}$ and $5.37\times10^{-9}$ S/m, respectively.

Complementary to conductivity characterization, we assessed the mechanical integrity of our interactive materials through flexural strength analysis. We conducted a three-point bending test across varying ratios of graphite and magnetite (see \textcolor{blue}{Section \ref{Flexural}} for details). We observe a slight marginal decline in flexural strength as the proportion of conductive fillers increased, as shown in \textcolor{blue}{Figure~\ref{fig:conductivity_implementation}b}.

For the decoding of conductivity, we implement the single-point bio-impedance sensing \cite{waghmare_z-ring_2023} using a vector network analyzer (VNA), the sensing setup is shown in \textcolor{blue}{Figure A\ref{fig:bioimpedance_setup}}. A VNA can transmit a signal into an antenna, subsequently analyzing the reflected signal to ascertain the antenna's impedance. This principle is adeptly applied to our context by channeling small (limit to 5 dBmW, safe for humans) radio frequency (RF) waves through a contact electrode into the user's finger. The impedance mismatch between the port and the finger causes a portion of the signal to reflect back. This mismatch, once the electrode establishes contact with the skin, becomes defined and relatively stable. Interaction with external conductive materials by the user introduces additional impedance variations as the signal extends flow from the sensor to these materials. By quantifying changes in the reflected signal, i.e., S11, we can identify the conductive interactive materials touched by the user.

During the real-world measurements, we positioned the electrode on the proximal phalange of the user's contact finger, to maintain consistency with our simulation protocols. The measurement is conducted under natural interactions, the interactive materials are placed across different substrates, such as wood and plastic tabletops, and the user can touch them at various pitch angles to simulate real-world usage scenarios of the interactive materials under diverse conditions, thereby stress-testing the robustness. The impedance sensor is configured to transmit signal sweeps ranging from 1 MHz to 500 MHz, executing 30 sweeps per second, and read 51 data points with each sweep.

The S11 parameter readings, collected from a single user but across different sections, exhibit a congruent trend with our theoretical deduction and EM simulation results, as shown in \textcolor{blue}{Figure~\ref{fig:conductivity_implementation}c}. Each conductive state shows a distinct impedance demarcation, offering good SNR.

The culmination of these efforts, the coherence presented from theoretical underpinnings to empirical validations, underscores the practicability of leveraging electrical properties as a medium for information encoding within materials and deploying wearable impedance sensors for decoding.

% The percolation threshold is a mathematical concept in percolation theory that describes the formation of long-range connectivity in random systems. 

==> sections/_Archive/v2_2_related_work.tex <==
\section{Related Work}

This interdisciplinary work builds on classic physics, sustainable materials, fabrications, sensing, and ubiquitous computing. There is no previous work similar to our proposed concept of \textit{interactive material} (IM). So we present the relevant works that motivated the goals of this work below, especially in computational materials \cite{abowd_internet_2020}.

\subsection{Internet of Materials}
Our initiative is motivated by the vision articulated by Gregory Abowd's vision talk at the UIST 2018, "Advances in materials science and manufacturing today signal a time when we really will be able to manufacture new everyday materials that have computational capabilities 'woven' into them". He introduced the notion of the Internet of Materials (IoM)  \cite{abowd_internet_2020} as an evolution beyond the well-known concept of the Internet of Things (IoT). He envisioned a future where "everyday objects made of everyday materials with the ability to behave as connected computational entities", these new and functional materials are termed "computational materials".

Despite the motivation and potential heralded by Abowd's vision, the reality, six years on, only a few works \cite{arora_saturn_2018,arora_mars_2021} meet his expectation for \textit{self-sustainable computational materials}. Most research had only focused on innovating the traditional IoT devices to be battery-free through the integration of energy-harvesting modules--- using photovoltaic or solar cells \cite{zhang_optosense_2020, zhang_flexible_2022, waghmare_ubiquitouch_2020, de_winkel_battery-free_2020}, piezoelectric generator \cite{lu_battery-less_2020, jang_underwater_2019}, or NFC \cite{kim_remote_2023} to replace conventional batteries. These works, while improved, fall short of achieving the transformative leap toward IoM.

The gap between the current state of technology and the envisioned future of IoM underscores the significant challenges involved in creating computational objects that simultaneously address self-sustainability in terms of power and life cycle, manufacturing scalability, and capability of mimicking the form factors of physical objects we interact with daily. It prompts a moment of reflection: Could we, perhaps, recalibrate our ambitions and explore the creation of interactive materials as a stepping stone toward computational materials?

\subsection{Internet of Bioinspired Things}
This reimagined approach is further inspired by the recent work on the Internet of Bioinspired Things \cite{iyer_wireless_2020, iyer_wind_2022, johnson_solar-powered_2023}, can we create interactive materials through the exploration of how nature’s entities, from honeybees to sea turtles and spiders, interact with their environment through innate mechanisms. These natural phenomena, although not "computational" in the sense of von Neumann architecture (used in today's modern computing and digital devices), offer rich ideas for our design of interactive materials (\textcolor{blue}{Figure~\ref{fig:overview}}).

\subsection{Sustainable Computing in HCI}
The urgency of sustainability permeates across disciplines, resonating strongly within the HCI community against the backdrop of the broader societal shift towards environmental consciousness. Yet, the path to ultimate sustainable computing is fraught with complexities, as evidenced by many recent works that used water-soluble plastic such as polyvinyl alcohol (PVA) \cite{cheng_functional_2023} but claimed "sustainable." However, these water-soluble plastics, while dissolving in water, do not disintegrate in the ecological sense; their chemical constituents persist, and complete biodegradation is contingent upon specific environmental conditions rarely met even in the wastewater treatment systems \cite{rolsky_degradation_2021}.

The most exciting research recently in sustainable computing has been directed toward the development of bio-based \cite{vasquez_myco-accessories_2019, koelle_prototyping_2022, nicolae_biohybrid_2023} and recyclable materials \cite{zhang_recyclable_2023} for circuits, aiming to extend the lifecycle of electronic components while circumventing the environmental pitfalls associated with processing the raw material of traditional bioplastics. Despite these advances, such biomaterials are often compromised by their inherent heterogeneity and non-cohesive morphologies, resulting in suboptimal mechanical properties and challenging processability issues, rendering them impractical for making everyday objects.

\subsection{Sensing for Interactive Surface}
Traditional sensing for surface interactions (e.g., touch detection) integrates sensors within physical interfaces, including capacitive \cite{sato_touche_2012, holloway_accessible_2018, cheng_swellsense_2023} and vibration sensors \cite{arora_saturn_2018, ding_surface_2023}. Beyond these, alternative strategies have explored the use of vision-based systems, mounting depth \cite{wilson_using_2010, xiao_direct_2016}, or thermal camera \cite{larson_heatwave_2011} above a given surface. These vision-based approaches, while powerful, often involve high setup costs and operational computational overheads for processing video data. Such requirements pose substantial barriers to the ubiquitous deployment of interactive surfaces into everyday environments, limiting their practicality.

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/Overview.png}
    \caption{The overview of our bio-inspired information encoding through natural material properties. 1) An off-of-shelf bioimpedance sensor can measure the impedance changes upon contact with an external conductive surface, akin to bees can perceive alterations in the electrical field surrounding flowers. 2) A common magnetometer can sense the shifts in the magnetic field upon nearing a magnetic surface, akin to turtles can discern the intensity and inclination of Earth's magnetic field for navigation. 3) An ubiquitous microphone can detect the vibrations induced by contact with an external tangible surface, akin to spiders can sense vibrations when prey touch their webs.}
    \label{fig:overview}
\end{figure*}

\section{Overview}
This section presents an overview of Biodegradable Interactive Materials, covering our selection of material properties for information encoding and curated list of sustainable materials, and the considerations underpinning our sustainable sensing design.

\subsection{Material Property Choice through Bioinspiration}
In the exploration of creating interactive materials through the lens of natural material property, our inspiration is drawn from the natural world (\textcolor{blue}{Figure~\ref{fig:overview}}). Animals have evolved various reception mechanisms to interact with or navigate nature.

\subsubsection{From Electroreception to Electrical Properties}
Honeybees, produce sensory hairs to perceive the electrical field surrounding flowers, so they can sense the alternation of the electric field surrounding flowers to determine if the flower has been recently visited, i.e., nectar availability before landing. This is because honeybees accumulate positive charges while flying while flowers gain negative charges through electrostatic induction, the interaction between honeybees and flowers alters the electric field of the flowers. Platypuses, also produce bills with electroreception to detect the electric fields generated by the muscular contractions of their prey. Such natural phenomena are highly attractive for creating interactive materials through electrical properties: can we leverage the natural electrical conductivity of materials as a medium for information encoding and sensing? 

\subsubsection{From Magnetoreception to Magnetism}
To expand the capabilities of interactive materials, our attention shifts towards magnetism. Drawing inspiration from the navigational prowess of sea turtles and migratory birds in the natural world, we delve into the potential of magnetism as a medium for encoding information. Sea turtles, for instance, utilize the Earth's magnetic field to discern their latitude during extensive migrations, relying on the field's intensity and inclination. Similarly, migratory birds harness directional cues from the magnetic field \cite{kishkinev_navigation_2021}, with cryptochrome in the eyes and magnetoreceptors in the beak region to perceive magnetic orientation and strength. These remarkable instances of bio-navigation by detecting tiny changes in magnetic intensity, combined with magnetic directional sense, present a compelling case for integrating magnetism into interactive materials.

\subsubsection{From Mechanoreception to Surface}
In our quest to expand the horizons of surface interaction through interactive materials, we now turn our attention back to the surface itself. In nature, where creatures such as spiders and rodents exhibit remarkable abilities to interact with their environment using surface properties: spiders, through their use of slit sensillae, a form of mechanical receptor capable of detecting minute vibrations and surface irregularities, excel in discerning varied terrains for web placement and vibrations traveling through their webs for prey hunting; rodents, with their highly sensitive whiskers, can also sense surface textures and shapes, enabling navigation and object identification in the dark. These biological mechanisms underline the potential of vibrations induced by surface properties and surface interactions as a rich medium for information encoding.

% Honeybees, produce sensory hairs to perceive the electrical field, so they can sense the alternation of the electric field surrounding flowers to determine if the flower has been recently visited, i.e., nectar availability; Sea turtles can detect magnetic field's intensity and inclination, so they utilize the Earth's magnetic field to discern their latitude; spiders have slit sensillae, a form of mechanical receptor capable of detecting minute vibrations and surface irregularities, so they can discern varied terrains for web placement and vibrations traveling through their webs for prey hunting. Such natural phenomena are highly attractive for creating interactive materials: can we leverage the natural physical property of every material as a medium for information encoding? 

\subsection{Sustainable Material Selection}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Biodegrade_Process_300ppi.png}
    \caption{Biodegradation in Soil. Photographs showing the biodegradation process of Biodegradable Interactive Materials disposed directly on backyard soil, the specimen is observably decomposed on Day 21. Note: on Day 7, a (white) centipede was eating the specimen (bottom-left).}
    \label{fig:biodegradation}
\end{figure*}

Addressing the limitations associated with traditional biomaterials, such as inferior mechanical properties and challenging processability, this work capitalizes on the recent advancements of creating backyard-compostable bioplastics from raw microalgae \cite{campbell_progress_2023}, with a simple and scalable fabrication methodology such as heat pressing \cite{iyer_fabricating_2023, liao_effects_2023} and 3D printing \cite{fredricks_spirulina-based_2021}. These techniques yield materials with mechanical properties comparable to those of conventional plastic filaments. As a proof of concept, we select chlorella (a type of edible algae; powder, Nuts, USA) as the base material, along with graphite (powder, Sigma Aldrich, USA) and magnetite Fe3O4 (a natural mineral; powder, Alpha Chemicals, USA) to tune the material properties. 

For the fabrication process for these biodegradable IMs, we first mix graphite or/and magnetite powder as filler in the chlorella matrix using a VWR Analog Vortex Mixer at varying weight percentages (0 wt\% for pure chlorella, and incrementally up to 28 wt\%). For the heat pressing process, the powder mixtures are compression molded in custom stainless steel molds on a TMAX-RT24D hot press at 15 MPa and 135 °C for 5 minutes, then a laser micromachining system (LPKF ProtoLaser U4) is used that scans its beam across the surface to pattern surface features and textures, with laser parameters carefully tuned to minimize the heat-induced carbonization to the material surface. For the 3D printing process, we mix the powder mixtures with deionized water at a weight ratio 1:1.2 (powder mixtures: water), then use a 3D Bioprinter (Direct-Ink-Writing; BioBot Basic, Advanced Solutions, USA) to print the powder mixtures, following by drying \cite{fredricks_spirulina-based_2021}. We note that while both fabrication methods prove effective, the heat pressing technique generally yields objects with superior mechanical integrity, attributable to the additional pressure applied during the process.

\paragraph{Biodegradation}
To demonstrate the backyard degradability of our IMs, we compost an IM (90 wt\% chlorella and 10 wt\% graphite) with featured laser-cut text in a yard located in the Northwestern United States 
% Seattle, Washington, USA
during the winter of 2024, spanning a duration of 21 days. The specimen was "disposed" directly on the soil surface, eschewing burial, to simulate a common disposal scenario. Daily weather conditions are recorded and detailed in \textcolor{blue}{Table A\ref{tab:biodegradation_daily_weather_data}} using the data from Weather Underground \footnote{\noindent\href{https://www.wunderground.com/}{https://www.wunderground.com/history/}}.
Photographic documentation captured the progressive decomposition of the IM over the trial period with discernable signs of decomposition, as shown in \textcolor{blue}{Figure \ref{fig:biodegradation}}. We note that many weather factors vary the degradation rates, for example, we found that dramatic shifts in temperature and humidity (e.g., a sunny day with a high UV index following a rainy day; day 7 to 8 and day 13 to 14) or persistent rain (day 17 to 21) would accelerate the degradation process.

We imagine the future of sustainable materials extracted from renewable biological matter and processed through eco-friendly techniques to minimize environmental burdens.

\subsection{Sustainability-driven Sensing Design Considerations}

\begin{table*}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/LCAComparison_Main_v2.png}
    \caption{Environmental impact comparison of our method (biodegradable interactive material + sensing on wearables) against conventional approaches of creating interactive surfaces. Our method has significant environmental benefit potential in the future world of ubiquitous interactive surfaces.}
    \label{tab:LCAComparison_Main}
\end{table*}

In addition to prioritizing sustainable materials, our design philosophy extends to optimizing sustainability in our sensing approach. 

The burgeoning IoT industry, with its exponential growth rate of billions of new devices every year \cite{daepp_eclipse_2022}, exemplifies the logistical and environmental challenges posed by embedded sensing mechanisms in physical interfaces. Such sensing approach for interactive material, while effective, risks compounding the already significant issue of e-waste. To circumvent these potential environmental repercussions, our strategy favors wearable device-based sensing. This choice is predicated on several advantages that align with sustainable practices: firstly, it centralizes the sensing mechanism, reducing the number of electronics per user to a single wearable device. This reduction is crucial for minimizing waste. Secondly, the personal nature of wearables facilitates better end-of-life treatment and power management, including the option to activate the device only when needed, thereby minimizing unnecessary power consumption power. 

Our cradle-to-grave environmental impact comparison in \textcolor{blue}{Table~\ref{tab:LCAComparison_Main}} (see \textcolor{blue}{Table A\ref{tab:LCAComparison_1}\&\ref{tab:LCAComparison_n}} for detailed comparisons of scenarios involving single and multiple interactive interfaces) juxtaposes our biodegradable interactive materials with the wearable-based sensing strategy against traditional methods involving 3D-printed physical interfaces equipped with embedded capacitive sensing circuits. This comparison leverages the recent concept in comparative life-cycle assessment (LCA) \cite{zhang_deltalca_2024} to underscore the environmental benefits of our approach.

In the subsequent sections, we delineate the creation of interactive materials utilizing three inherent material properties. An overview of these material properties and their associated sensing technologies is illustrated in \textcolor{blue}{Figure~\ref{fig:overview}}. For each material property explored, we leverage commonly available sensors (e.g., impedance sensors, magnetometers, microphones) for information decoding. This decision to utilize off-the-shelf sensors, rather than developing custom sensors, is informed by two practical considerations that may throttle the pace of further innovation in interactive material: 1) custom sensors often incur prohibitive fabrication costs and times \cite{wang_neuromorphic_2023}, making replication inaccessible to researchers in the broader HCI community; 2) sensors tailored for specific purposes may have difficulty adapting to new material properties or scenarios.

Through these considerations, our approach not only adheres to our principles of sustainable computing but also paves the way for the ubiquitous deployment of interactive materials.

==> sections/_Archive/v2_3_conductivity.tex <==
\section{Electrical Encoding and Sensing}
% In the exploration of creating interactive materials through the lens of conductivity, our inspiration is drawn from the natural world. Animals have evolved various mechanisms to use electroreception to interact with or navigate nature. Platypuses, produce bills with electroreception to detect the electric fields generated by the muscular contractions of their prey; honeybees, produce sensory hairs to perceive the electrical field surrounding flowers. Honeybees accumulate positive charges while flying while flowers gain negative charges through electrostatic induction. The interaction between honeybees and flowers alters the electric field of the flowers, this alteration, with information about the flower has been recently visited, i.e., nectar availability could be perceived by other honeybees before landing. Such natural phenomena are highly attractive for creating interactive materials: conductivity could not just be a physical property but a medium for information encoding and sensing. 

Building on our inspiration from the electroreception of honeybees, in this section, we aim to encode information into materials through conductivity and extend human sensory capabilities by leveraging the recent development of wearable bio-impedance sensing technology \cite{waghmare_z-ring_2023, zhang_advancing_2016, jung_wrist-wearable_2021}. Our approach aims to replicate, in human users, a bee-like ability to discern and interact with the electrical properties of their surroundings. 

\subsection{Theory}
The foundational premise of employing material conductivity $\sigma$ to encode information and its decoding through wearable bio-impedance sensors is rooted in an amalgam of classical electrical theory and contemporary bioelectrical impedance analysis. We explain the backbone of this conceptual framework using elements of a simplified circuit model that encapsulates the interaction between the user and the interactive materials. 

We assume that the user's finger and the external surface form a series connection upon contact, the system's total impedance, $Z_{total}$, manifests as the sum of the finger's bio-impedance $Z_{bio}$, the contact electrical impedance $Z_{contact}$, and the inherent material impedance $Z_{material}$, mathematically represented as:
\begin{equation}
   Z_{total} = Z_{bio} + Z_{contact} + Z_{material}
\label{eq:Z_total}
\end{equation}

Bio-impedance, a measure of biological tissues' opposition to electric current, varies with tissue type and state, such as hydration. In our case, we neutralize the variable of the user's inherent bio-impedance by only focusing on the change in impedance $\Delta Z$ upon contact with an external surface, i.e., the add-in impedance of interactive material and contact:
\begin{align}
    \Delta Z &= Z_{total,new} - Z_{total,initial} \nonumber \\
    \Rightarrow \Delta Z &= (Z_{bio} + Z_{contact} + Z_{material}) - Z_{bio} \nonumber \\
    &= Z_{contact} + Z_{material}
\label{eq:delta-Z}
\end{align}

\subsubsection{Contact Impedance}
Our theoretical framework made the following simplifying assumptions:
\begin{enumerate}
    \item Contact surfaces are clean without insulating barriers, as well as continuous and frictionless.
    \item There is no tensile stress at the contact point.
    \item User's finger is a perfectly elastic solid and skin surface is smooth, i.e., no friction ridges and lines; external interactive material surface is a perfectly rigid body.
\end{enumerate}

Under these conditions, $Z_{contact}$ is governed by the resistivity, and the size of the contact radius relative to the electron mean free path, which transitions between Sharvin and diffuse scattering mechanism, as explained in the Maxwell spreading resistance formula \cite{wexler_size_1966}:
\begin{equation}
    Z_{contact} = \frac{4\rho^{*} l_{e}}{3\pi a^{2}} + v\left(l_{e}/a\right)\frac{\rho^{*}}{2a}
\label{eq:Wexler}
\end{equation}
where $\rho$ is the resistivity separating two bodies, $l_{e}$ is the electron mean free path length of the material, $a$ is the contact radius, $v$ is a function of the ratio $l_{e}/a$, and $\rho^{*}$ is $\frac{\rho_1+\rho_2}{2}$, $\rho_1, \rho_2$ are the resistivity on two sides of the contact, respectively. Given the dominance of the diffuse scattering mechanism in our context $a \gg l_{e}$, so that
\begin{align}
    \lim\limits_{{l_e}/a \to 0} v\left({l_e}/a\right) &= 1 \nonumber \\
    \frac{4\rho^{*} l_{e}}{3\pi a^{2}} &\approx 0 \nonumber 
\label{eq:le/a}
\end{align}
Now Eq.\ref{eq:Wexler} can be simplified to
\begin{equation}
    Z_{contact} = 0 + 1\times\frac{\rho^{*}}{2a} = \frac{\rho^{*}}{2a} \Leftrightarrow \frac{\rho_{finger}+\rho_{material}}{4a}
\label{eq:Wexler_simplified}
\end{equation}

This relationship is further refined through the Hertzian contact stress model, accounting for the applied force and the elastic properties of the finger and interactive material, to express the effective contact radius of the finger pad $a$ and, consequently, the contact area $A$. For contact radius $a$, we arrive at a simplified Hertzian contact stress model (refer to \textcolor{blue}{Section \ref{Detailed_HertzianContactStressModel}} for detailed derivation) as

\begin{equation}
    a = \left[ \frac{9F R_{finger}} {16 \left( \frac{E_{finger}}{1-{v_{finger}}^{2}} \right)} \right]^{\frac{1}{3}}
\label{eq:Hertzian_final}
\end{equation}
where $F$ is the force applied over the contact area of the finger and material surface, $R_{finger}$, $E$, $v$ are the effective radius of curvature, elastic modulus, and Poisson's ratio of the finger, respectively.

% \begin{equation}
%     A = \pi a \xi = \pi\left[ \frac{9FR_{finger}} {16 \left( \frac{E_{finger}}{1-{v_{finger}}^{2}} \right)} \right]^{\frac{2}{3}}
% \label{eq:contact_area }
% \end{equation}

In validating our theoretical contact stress model of the finger and interactive material, empirical results from recent studies characterizing human skin tissue and finger mechanics are used: a Poisson ratio for human skin tissue of 0.48 \cite{li_determining_2012}; an average tap force of 0.50 N with a standard deviation of 0.09 N \cite{asakawa_fingertip_2017}; the elasticity of the finger, as characterized by Young’s modulus, presents a wide range due to factors such as applied normal load, gender differences, and the anatomical variance between the skin's superficial and deeper layers adjacent to the bone, fluctuating between 0.2 MPa \cite{oprisan_experimental_2016} and 4.6 MPa \cite{pawlaczyk_age-dependent_2013}. For the purposes of our analysis, the effective curvature radius of the finger is approximated as 1 cm. Substituting these empirically derived values into our final Hertzian contact stress model Eq.\ref{eq:Hertzian_final}, we derive the effective contact radius: 
\begin{align}
    % a &= \left[ \frac{9\cdot0.5N\cdot0.01m} {16 \left( \frac{E_{finger}}{1-{0.48}^{2}} \right)} \right]^{\frac{1}{3}}, E_{finger}\in [0.2 MPa, 4.6 MPa] \nonumber \\
    a &\in [0.84 mm, 2.40 mm]
\label{eq:radius_number}
\end{align}

These results align with empirical observations---19.9 and 14.0 mm for the orientations of 30° and 45° \cite{dzidek_contact_2017}. This stress model is a critical component in understanding the contact interface of tactile interactions and the simulation in the subsequent section. A study also characterized the resistivity of the living epidermis (the outermost layer of skin) of fingers to be 11 $\Omega \text{m}$ at 1 MHz \cite{tsai_dielectrical_2019}. By integrating these datums into Eq.\ref{eq:Wexler_simplified}, we derive the contact impedance, $Z_{contact}$, as a function of material resistivity:

\begin{equation}
    Z_{contact} = \frac{11 \Omega \text{m}+\rho_{material}}{4a}, a \in [0.84 mm, 2.40 mm]
\label{eq:Wexler_final}
\end{equation}

\subsubsection{Impedance of Interactive Material}

The intrinsic impedance $Z_{material}$ diverges in behavior under alternating current (AC) conditions, necessitating a distinction from direct current (DC) scenarios where impedance equates to resistance, $R$. In the AC paradigm, where common capacitive sensors and bio-impedance sensors operate at, $Z_{material}$ embodies both resistive and reactive components:
\begin{equation}
    Z_{material} = R+jX
\label{eq:Z_material}
\end{equation}
where $j$ is the imaginary unit and $X = \omega L - \frac{1}{\omega C}$, $\omega$ is the angular frequency $2\pi f$. Assume interactive materials as regular solid cuboids with constant area $A$ and thickness $t$ for simplification, we deduce expressions for resistance, $R = \rho \frac{t}{A}$, and capacitance, $C = \frac{t}{\omega \epsilon A}$. Due to the diamagnetism of common conductive materials such as copper, silver, and graphite, which results in low magnetic permeability, the inductance part could be negligible. Now we have Eq.\ref{eq:Z_material} as
\begin{equation}
    Z_{material} = \rho \frac{t}{A} - j\frac{t}{\omega \epsilon A} = \frac{t}{A} (\rho - j\frac{1}{\omega \epsilon})
\label{eq:Z_material_2}
\end{equation}

We know that in the theory of wave causality in classical electrodynamics, permittivity is a complex quantity and can be expressed as $\epsilon = \epsilon' + j\epsilon'' = \epsilon_0 + j \frac{\sigma}{\omega } \Rightarrow j\frac{1}{\omega \epsilon} = j\frac{1}{\omega  (\epsilon_0 + j \frac{\sigma}{\omega })} = \frac{-\omega }{j\omega^2 \epsilon_0 - \sigma}$. Thus, Eq.\ref{eq:Z_material_2} arrives at:

\begin{equation}
    Z_{material} = \frac{t}{A} (\frac{1}{\sigma} + \frac{\omega }{j\omega^2 \epsilon_0 - \sigma})
\label{eq:Z_material_3}
\end{equation}

\subsubsection{Final Impedance Change Model}
For the minimal dimensions of interactive material pixel, we adhere to Apple’s Accessibility Human Interface Guidelines \cite{apple_accessibility_nodate}, which suggest that a hit target should measure at least 44$\times$44 points, approximately 15$\times$15 mm. We envision our interactive materials being applied to the surface of everyday objects rather than filling the entire solid object. Consequently, they will be thin, such that $t\ll A$. Therefore, the impedance of the interactive material is negligible in our final calculation unless in a low-frequency region (e.g., $f<1kHz$), where the term $(\rho - \frac{1}{\omega \epsilon})$ is dominated by the permittivity. We thereby describe the impedance change Eq.\ref{eq:delta-Z} as: 
\begin{align}
     \Delta Z &= Z_{contact} + Z_{material} \approx Z_{contact} \nonumber \\
     &= \frac{11 \Omega \text{m}+\rho_{material}}{4a}, a \in [0.84 mm, 2.40 mm], f > 1MHz
\label{delta-Z-final}
\end{align}

% To ensure a good SNR or read margin between each possible conductivity state, we consider the varies in such as touch force and tissue properties between each touch and user as background noise or the region of uncertainty. We use the measured resistivity of chlorella ($1.86\times10^8 \Omega \text{m}$) as the upper bound (please refer to the subsequent section) and $\rho_{finger}$ ($11 \Omega \text{m}$) as the lower bound for the possible tuning range of $\rho_{mateiral}$, this is because if the interactive material has great conductivity, i.e., $\rho_{mateiral} \ll \rho_{finger}$, the contact resistance part will be dominated by $\rho_{finger}$. In that case, we could tune the size $A$ of the interactive material to encode information. However, surface pattern is a different property that will not be discussed in the section. Such that, by tuning the material conductivity, we are able to encode 

To optimize the signal-to-noise ratio (SNR) and read margin between each possible conductivity states, the variance in touch force and user-specific biological tissue properties are considered as background noise or the uncertainty region. We set the resistivity bounds of $\rho_{mateiral}$ from $1.86\times10^8 \Omega \text{m}$ (the resistivity of chlorella, see resistivity measurement in \textcolor{blue}{Section \ref{conductivity_implementation}}) to $\rho_{finger}$ $11 \Omega \text{m}$. This delineation is predicated on the principle that if the interactive material exhibits superior conductivity like copper (i.e., $\rho_{material} \ll \rho_{finger}$), then the contact resistance part will be dominated by $\rho_{finger}$. Under such circumstances, the dimension—specifically, the area ($A$) of the interactive material—becomes a tunable parameter for encoding information, however this is a different material property and will not be discussed here. In conclusion, by tuning the conductivity of the material, it becomes feasible to encode information within a spectrum of approximately 32 discrete states, equivalent to 5 bits of data, as expressed by the following equation:

\begin{equation}
    \log_{1.68}{(1.86\times10^8 \Omega \text{m} \div 11 \Omega \text{m})} \approx 32 \text{ states} \Leftrightarrow \log_{2}{32} = 5 \text{ bits}
    \label{eq:conductivity_result}
\end{equation}

Through this theoretical exposition, our objective is not only to elucidate the boundaries of information encoding within materials via conductivity but also to outline the mechanism by which a wearable impedance sensor could decode this information.

% S11:
% \begin{equation}
%     S11 = \frac{Z_{L} - Z_{0}}{Z_{L} + Z_{0}}
% \label{eq:s11}
% \end{equation}

\subsection{Simulation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Conductivity_simulation_v2.png}
    \caption{Electrical Simulation. a, Simulation setup of conductive interactive material and bio hand model in CST Studio Suite, as well as pitch angle offset setup and the cross-section of bio hand model showing various body tissues. b, Simulated S11 results, showing the amount of signal reflected caused by impedance mismatch resulting from contact with external surfaces with corresponding conductive levels. c, Simulated S11 results respond to varying pitch angle offsets.}
    \label{fig:conductivity_simulation}
\end{figure*}

Before transitioning from theory to real-world validations, the employment of FIT simulation is an indispensable intermediary in the iterative design process, as it provides a controlled environment to test our hypotheses regarding material conductivity and its decoding through wearable impedance sensors.

In our specific study, the simulation is conducted using the Simulia CST Studio Suite, leveraging its 3D electromagnetic (EM) analysis capability. We determine the frequency range of 1 MHz to 500 MHz for our simulations, drawing on recent findings highlighting a significant attenuation of specific absorption rate (SAR) dynamics within human tissue beyond 500 MHz \cite{waghmare_z-ring_2023}.

We constructed a bio hand model representative of a 38-year-old male, 180 cm in height and 103 kg in weight, utilizing the CST Bio Models Library and the US National Library of Medicine's Visible Human Project. Our model incorporates 31 distinct tissue types at a resolution of $1\times1\times1 \text{mm}$, and isolates the right hand from the rest of the body tissues to reduce the size of mesh volume and computation complexity. The bio-impedance measurement point is set at the proximal phalange (the common position to wear a ring-form-factor device) of the index finger (the common finger to touch an external object). 

The interactive materials are created with dimensions of $20\times20\times5 \text{mm}$, balancing the requirements for minimal accessible touch size and interactive material 'pixel' density. Within this framework, conductivity emerges as the sole variable, with all other material properties, such as loss tangent, held constant to isolate the effect of other contributions. The simulation models the contact interface between the fingerpad and interactive materials, following our calculation in Eq.\ref{eq:radius_number} of contact radius and pressure distribution. The final model setup is illustrated in \textcolor{blue}{Figure~\ref{fig:conductivity_simulation}a}.

To explore the conductivity spectrum of the interactive materials, we conduct a logarithmic parameter sweep from $5.37\times10^{-9}$ S/m to $6.87\times10^{-7}$ S/m with a total of 8 samples. This interval selection is predicated on the minimal read margin calculated in Eq.\ref{eq:conductivity_result} to achieve a good SNR, ensuring discernible differentiation between each conductive state. Each parameter value required approximately 100 minutes for simulation on a 14-core CPU and a single RTX 4070Ti GPU. The measurements of S11, also known as the reflection coefficient, are used to determine the impedance. S11 is a metric that specifies the amount of a wave reflected by the impedance mismatch in the transmission medium, defined as the ratio of the reflected wave’s amplitude to the incident wave’s amplitude. The simulation results reveal macroscopic distinctions across 8 conductivity levels as shown in \textcolor{blue}{Figure~\ref{fig:conductivity_simulation}b}, corroborating our theoretical predictions.

Further examination extends to the influence of finger orientation on touch interaction. We perform another linear parameter sweep of touch pitch angles from -20 degrees to +20 degrees with a total of 5 samples onto the existing model. The S11 simulation results, along with the nearest conductivity states as references, are shown in \textcolor{blue}{Figure~\ref{fig:conductivity_simulation}c}, revealing the robustness of conductivity detection across a range of touch orientations. The aggregation of these 3D EM simulation results validates our theoretical constructs.

%https://space.mit.edu/RADIO/CST_online/mergedProjects/3D/common_tools/common_tools_biomodels.htm


\subsection{Implementation} \label{conductivity_implementation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Conductivity_measurement.png}
    \caption{Electrical Implementation. a,b, Characterized conductivity (a) and flexural strength (b) of Interactive Materials with different proportions of graphite and magnetite, data is presented as mean (SD) of 3 (a) and 9 (b) specimens in 1000 (a) and 1 (b) measurements of each proportion. c, Measurements from a wearable bioimpedance sensor when user's finger is in contact with external surfaces of corresponding conductive states ($N=2\times5\times2\times30=600$ frequency sweeps per state, shaded region indicates SD).}
    \label{fig:conductivity_implementation}
\end{figure*}

Having substantiated our hypothesis through both theoretical articulation and simulation insights, we now transition to the tangible implementation. This phase entails the fabrication of interactive materials with varied conductivities, alongside the development of a wearable sensor system capable of decoding this conductivity. We aim to validate the feasibility of our approach in encoding information within materials through their inherent conductivity properties in practice.

We fabricate the interactive material with different conductivities by mixing chlorella with varying proportions (0\%--28\%) of graphite or magnetite Fe3O4. Graphite, is a crystal allotrope of carbon, exhibiting good electric conductivity due to the delocalized $\pi$-electrons between carbon hexagonal lattice layers; Magnetite, a natural mineral of iron ores, exhibits electrical conductivity attributed to electron exchange between iron ions in different oxidation states within the crystal lattice.

We first characterize the conductivity of the fabricated samples (see \textcolor{blue}{Section \ref{Conductivity}} for details), revealing a direct positive correlation between the addition of conductive materials and enhanced conductivity. The results are shown in \textcolor{blue}{Figure~\ref{fig:conductivity_implementation}a}. We note that graphite's inclusion resulted in a more pronounced increase in conductivity compared to magnetite, reflective of its superior electrical properties (graphite: $3.3\times10^2$ to $2\times10^5$ S/m, magnetite: 0.1 S/m). We observe a stark rise in conductivity between graphite concentrations of 5\% to 8\%, marking the percolation threshold--- a point at which our interactive material transitions from a nearly insulator to a conductor due to the formation of a continuous path for electron flow. The resistivity and conductivity of pure chlorella are characterized at $1.86\times10^8 \Omega \text{m}$ and $5.37\times10^{-9}$ S/m, respectively.

Complementary to conductivity characterization, we assessed the mechanical integrity of our interactive materials through flexural strength analysis. We conducted a three-point bending test across varying ratios of graphite and magnetite (see \textcolor{blue}{Section \ref{Flexural}} for details). We observe a slight marginal decline in flexural strength as the proportion of conductive fillers increased, as shown in \textcolor{blue}{Figure~\ref{fig:conductivity_implementation}b}.

For the decoding of conductivity, we implement the single-point bio-impedance sensing \cite{waghmare_z-ring_2023} using a vector network analyzer (VNA), the sensing setup is shown in \textcolor{blue}{Figure A\ref{fig:bioimpedance_setup}}. A VNA can transmit a signal into an antenna, subsequently analyzing the reflected signal to ascertain the antenna's impedance. This principle is adeptly applied to our context by channeling small (limit to 5 dBmW, safe for humans) radio frequency (RF) waves through a contact electrode into the user's finger. The impedance mismatch between the port and the finger causes a portion of the signal to reflect back. This mismatch, once the electrode establishes contact with the skin, becomes defined and relatively stable. Interaction with external conductive materials by the user introduces additional impedance variations as the signal extends flow from the sensor to these materials. By quantifying changes in the reflected signal, i.e., S11, we can identify the conductive interactive materials touched by the user.

During the real-world measurements, we positioned the electrode on the proximal phalange of the user's contact finger, to maintain consistency with our simulation protocols. The measurement is conducted under natural interactions, the interactive materials are placed across different substrates, such as wood and plastic tabletops, and the user can touch them at various pitch angles to simulate real-world usage scenarios of the interactive materials under diverse conditions, thereby stress-testing the robustness. The impedance sensor is configured to transmit signal sweeps ranging from 1 MHz to 500 MHz, executing 30 sweeps per second and reading 51 data points with each sweep. The S11 parameter readings collected cross-session from a single user (each session consisted of 5 repetitions of each conductive state, and each repetition consisted of 1 measurement of 2-second duration), exhibit a congruent trend with our theoretical deduction and EM simulation results, as shown in \textcolor{blue}{Figure~\ref{fig:conductivity_implementation}c}. Each conductive state shows a distinct impedance demarcation, offering good SNR.

The culmination of these efforts, the coherence presented from theoretical underpinnings to empirical validations, underscores the practicability of leveraging electrical properties as a medium for information encoding within materials and deploying wearable impedance sensors for decoding.

% The percolation threshold is a mathematical concept in percolation theory that describes the formation of long-range connectivity in random systems. 
